R&D Proposal, RD51 Extension Beyond 2018

The RD51 Collaboration, in charge of the development and dissemination of MicroPattern Gaseous Detectors (MPGD) since 2008, proposes to extend its activity, after 2018, for a further five-year term. Since the RD51 initial years, the community of MPGD developers and users has grown considerably. It is reflected by the many MPGD-based applications in high energy and nuclear physics experiments as well as in other basic and applied-research fields. They rely on the parallel progress of detector concepts and associated technologies. The cultural, infrastructure and networking support offered by RD51 has been essential in this process. The rich portfolio of MPGD projects, under constant expansion, is accompanied by novel ideas on further developments and applications. The proposed next term of RD51 activities aims at bringing a number of detector concepts to maturity, initiating new projects and continuing the support to the community. Among leading proposed projects are ultrafast, high-rate MPGDs; discharge-free, high-resolution imaging detectors with resistive elements and high-granularity integrated electronics; novel noble-liquid detector concepts, including electroluminescence in gas bubbles; studies of environment-friendly counting gases and long-term sealed-mode operation; optical-readout detectors with radiation-hard imagers for fundamental research experiments, radiography and other domains. The proposed R&D program is also expected to enrich our basic knowledge in detector physics, to form a generation of young detector experts - paving the way to new detector concepts and applications. The vast R&D program requires acquiring additional, up-to-date expertise in advanced technologies.

==> executive_temporary.tex <==
The RD51 Collaboration, in charge of the development and dissemination
of Micro-Pattern Gaseous Detectors (MPGD) since 2008, proposes to extend
its activity, after 2018, for a further five-year term. This proposal, 
where the Collaboration community expresses firm interest, 
is based on the analysis of the progress in the MPGD sector during 
the RD51 years and the Collaboration contribution to the 
present status of the art; on the legacy in terms 
of expertize and infrastructures that RD51 has built-up over years; 
on the perspectives for future R\&D projects and the wide dissemination 
of MPGD usage, where the Collaboration can continue offering relevant
cultural and infrastructural support. Therefore, 
the scope and activities for the RD51 extension cluster around 
two main missions: novel R\&D developments towards reaching or breaking performance limits and the continuation and reinforcement of  the
support actions for the community and the MPGD dissemination.
\par
Highlights of the future R\&D scenario based on the ongoing projects  
are central elements of the present proposal. A clear direction 
for future developments is that of the resistive  materials 
and related detector architectures. Their usage improves 
detector stability, making possible higher gain in a single 
multiplication layer, a remarkable advantage for assembly, 
mass production and costs. 
Single layer 
architectures represent also a preferential approach in
hadron sampling calorimetry. 
\par
The frontier of fast and precise 
timing is moved forward by developments as the PICOSEC one, where gaseous 
detectors are coupled to Cherenkov radiator to take advantage 
from the prompt radiation emission. Correspondingly novel electronics and 
front-end circuits are being developed.
\par 
A variety of novel opportunities is offered by MPGD hybridization, 
both combining MPGD technologies to strength the performance and 
coupling gaseous detector to different detection technologies, 
as it is the case for optical read-out of gaseous detectors.
\par 
Contributions to the detector concepts from up-to-date material science 
is required concerning resistive materials, solid-state photon 
and neutron converters, 
innovative nanotechnology components. Material studies can 
contribute to requirements related to low out-gassing, 
radiation hardness, radio 
purity, converter robustness and eco-friendly gases.
\par 
The support actions towards the community is aimed to preserve 
and enrich the present scenario, including: 
networking activity, with focus on training and education, 
further development of dedicated simulation tools, 
advances in electronics tools, continuation of the
collaborative interactions 
with strategic CERN workshops. The need of  new materials 
and technologies
will result in an RD51 action of stimulus to the whole
community of detector developers towards the creation of 
common networking and infrastructures.
\par
The collaboration plans to maintain the current organization, 
characterized by a simple and effective management,
and the existing structure based on the  working groups.
\par 
The Collaboration requests to CERN are moderate and at a level similar 
to the present one, with emphasis to the support of the Gaseous Detector
Development (GDD) laboratory, the collaborative access to 
the EP-DT-EF MPT (Micro Pattern Technology) Workshop and to 
the EP-DT-EF TFG (Thin Film and Glass) Laboratory, as well 
as access to other CERN technical facilities.

==> references_extension.tex <==

\bibitem{LAPPD} Large-Area Picosecond Photo-Detectors Project\\ \url{https://psec.uchicago.edu/}

\bibitem{FAST} Fast Advanced Scintillator Timing\\ \url{http://fast-cost.web.cern.ch/fast-cost/}

==> short_abstract_initialSilvia.tex <==
The RD51 Collaboration, at work to facilitate the development and dissemination
of MicroPattern Gaseous Detectors (MPGD) since 2008, proposes to continue
its activity for a further five-year term after 2018. Since 2008, the community of
MPGD users has greatly enlarged with corresponding wide usage dissemination in
the high energy physics experiments, in other scientific fields and in sectors beyond
fundamental research, accompanied by technological progress, novel architectures
and development of dedicated tools. The cultural, infrastructural and networking
support offered by RD51 has represented an essential ingredient in this process.
The expansion of the MPGD developments and applications is still ongoing, while
a rich portfolio of R\&D projects and novel ideas is present.
\par
The next term of RD51 activities is dedicated to bring a number of new projects
to maturity, while continuing the support to the wide community along the same
guide-lines and strategies already implemented. The main future R\&D focus is
on the development of MPGD with unprecedented fine time resolution by the detection
of Cherenkov light or secondary emission, with extremely high rate capabilities
by mastering the use of resistive elements in the MPGD architecture, with
extremely fine space resolution by increased granularity with integrated electronics,
on studies dedicated to gases to match environmental requirements, seal operation
requirements and increased detector lifetime, on the extension of the optical readout
approach by radiation hard imagers in order to open this concept to the use
in high energy physics experiments. The whole R\&D program requires important
enrichments in up-to-date technological know-how.

==> short_abstract_old.tex <==
The RD51 Collaboration, in charge of the development and dissemination 
of MicroPattern Gaseous Detectors (MPGD) since 2008, proposes to 
extend its activity, after 2018, for a further five-year term. 
Since 2008, the community of MPGD developers and users has grown considerably. It is reflected by the many MPGD-based applications 
in high energy and nuclear physics 
experiments as well as in other basic and applied-research fields. 
The remarkable progress in detector concepts has relied on a parallel 
one, on associated technologies and construction methods. The cultural, infrastructural and networking support offered by RD51 has  
been essential in this process. The rich portfolio of MPGD 
projects, under constant expansion, is accompanied by novel 
ideas on further developments and applications.
\par
The proposed next term of RD51 activities aims at bringing a number 
of detector  concepts to maturity, initiating new projects and 
continuing the support to the community. Among leading proposed 
projects are ultrafast, high-rate MPGDs  based on Cherenkov-light 
and secondary-emission detection;  discharge-free, high-resolution 
imaging detectors with resistive elements and high-granularity 
integrated electronics; novel noble-liquid detector concepts, 
including electroluminescence in gas bubbles; studies of 
environment-friendly 
counting gases and long-term sealed-mode operation; optical-readout
detectors with radiation-hard imagers for HEP experiments 
and radiography and more.
\par
The proposed R\&D program is also expected to enrich our basic knowledge 
in detector physics, to form a generation of young detector 
experts - paving the way to new detector concepts and applications. 
The whole R\&D program requires important  enrichments 
in up-to-date technological know-how.

